Fast and Accurate: Video Enhancement using Sparse Depth

This paper presents a general framework to build fast and accurate algorithms for video enhancement tasks such as super-resolution, deblurring, and denoising. Essential to our framework is the realization that the accuracy, rather than the density, of pixel flows is what is required for high-quality video enhancement. Most of prior works take the opposite approach: they estimate dense (per-pixel)-but generally less robust-flows, mostly using computationally costly algorithms. Instead, we propose a lightweight flow estimation algorithm; it fuses the sparse point cloud data and (even sparser and less reliable) IMU data available in modern autonomous agents to estimate the flow information. Building on top of the flow estimation, we demonstrate a general framework that integrates the flows in a plug-and-play fashion with different task-specific layers. Algorithms built in our framework achieve 1.78x - 187.41x speedup while providing a 0.42 dB - 6.70 dB quality improvement over competing methods.

==> method.tex <==
\section{Main Idea}
\label{sec:idea}

\begin{figure}[t]
%\vspace{-8pt}
\centering
\includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{idea}
\caption{The algorithm of LiDAR-guided motion estimation. $P^*$ is the 3D coordinates of a point in the LiDAR coordinate system in Frame $t$. $T_{lidar2cam}$ is the transformation matrix from the LiDAR coordinate system to the camera coordinate system. $T_cam$ is the camera matrix. $T_{cam2cam}$ is the camera transformation matrix from Frame $t$ to Frame $t+1$.}
\label{fig:idea}
%\vspace{-8pt}
\end{figure}

The key idea is to use the depth data from LiDAR to generate motion in a lightweight fashion. \Fig{fig:idea} illustrates the idea. For any point $P^*$ in a point cloud, it is captured by two consecutive camera frames. The offset between the corresponding pixels in the two frames is the motion.

For each point $P^*$ in the point cloud at time $t$, its coordinates in the camera coordinate system at $t$ is $P = P^* \times T_{lidar2cam}$, where $T_{lidar2cam}$ is the LiDAR to camera transformation matrix, which is usually pre-calibrated. Thus, the corresponding pixel coordinates in the image at time $t$ is $P_t = T_{cam} \times P$, where $T_{cam}$ is the camera matrix.

At time $t+1$, the coordinates of the same point in the scene can now be expressed in terms of the camera coordinate system at $t+1$ as $T_{cam2cam} \times P$, where $T_{cam2cam}$ is the camera transformation. Thus, the pixel coordinates of the point at $t+1$ is $P_{t+1} = T_{cam} \times T_{cam2cam} \times P$.

Assuming that the point does not move between time $t$ and $t+1$, we can tell that pixel $P_t$ in Frame $t$ and pixel $P_{t+1}$ in Frame $t+1$ match, allowing us to calculate the motion of $P_t$.

The camera transformation could be derived in a range of different methods, such as directly reading from the IMU that is readily available in virtually all intelligent devices (e.g., robotics, autonomous vehicles, smartphones) or through computational techniques such as point cloud registration~\cite{??}. Computational methods are generally known to be more accurate than the reading from consumer-grade IMUs~\cite{??}. A key contribution of our paper is to show that even with relatively less accurate camera transformation from an IMU, our algorithm can still yield higher task accuracy while greatly reducing the execution time.













